Separability in B\"uchi Vass and Singly Non-Linear Systems of Inequalities

The omega-regular separability problem for B\"uchi VASS coverability languages has recently been shown to be decidable, but with an EXPSPACE lower and a non-primitive recursive upper bound -- the exact complexity remained open. We close this gap and show that the problem is EXPSPACE-complete. A careful analysis of our complexity bounds additionally yields a PSPACE procedure in the case of fixed dimension >= 1, which matches a pre-established lower bound of PSPACE for one dimensional B\"uchi VASS. Our algorithm is a non-deterministic search for a witness whose size, as we show, can be suitably bounded. Part of the procedure is to decide the existence of runs in VASS that satisfy certain non-linear properties. Therefore, a key technical ingredient is to analyze a class of systems of inequalities where one variable may occur in non-linear (polynomial) expressions. These so-called singly non-linear systems (SNLS) take the form A(x).y >= b(x), where A(x) and b(x) are a matrix resp. a vector whose entries are polynomials in x, and y ranges over vectors in the rationals. Our main contribution on SNLS is an exponential upper bound on the size of rational solutions to singly non-linear systems. The proof consists of three steps. First, we give a tailor-made quantifier elimination to characterize all real solutions to x. Second, using the root separation theorem about the distance of real roots of polynomials, we show that if a rational solution exists, then there is one with at most polynomially many bits. Third, we insert the solution for x into the SNLS, making it linear and allowing us to invoke standard solution bounds from convex geometry. Finally, we combine the results about SNLS with several techniques from the area of VASS to devise an EXPSPACE decision procedure for omega-regular separability of B\"uchi VASS.

==> prelim_buechi.tex <==
\newcommand{\ekmark}[1]{\color{purple}#1\color{black}~}
\newcommand{\loopvector}{\mathbf{o}}
\newcommand{\valuevec}{\bz}
\newcommand{\countersp}{J}
\newcommand{\pathsof}[1]{\mathsf{path}(#1)}
\newcommand{\reachof}[2]{\mathsf{reach}(#1.#2)}
\newcommand{\runreachesof}[1]{\mathsf{reach}(#1)}


\section{B\"uchi VASS}

To adequately formulate our proofs, we need to introduce some more VASS-related concepts.

Let $\avass=(Q, q_0, \Sigma, T, F)$ be a B\"uchi VASS.
%
Consider a (possibly infinite) run 
$\sigma=(p_0, \bmm_{0})\xrightarrow{w_1}(p_1, \bmm_1)\xrightarrow{w_2}\cdots$ of $\avass$.
%
%
%
%
The underlying sequence of transitions of $\sigma$ is called a \emph{path} and has the form
$\apath=(p_0, w_1, \delta_1, p_1)(p_1, w_2, \delta_1, p_2)\ldots$.
%
We denote the set of all paths in $\avass$ by $\pathsof{\avass}$.
%
If a path is finite and the source state of its first transition coincides with the target state of its last transition, we call it a \emph{loop}, and denote the respective set by $\loopsof{\avass}$.

Since a run is uniquely determined by the starting configuration and the sequence of transitions taken from it, we also write $\sigma=(p_0, \bmm_{0}).\apath$ to denote a run.
%
For a finite run $\sigma$, we write $\runreachesof{\sigma}$ to denote the last configuration it reaches.
%
It is also useful to define the \emph{effect} of a path.
%
The effect $\vassbalanceof{\apath}$ of some finite $\apath=(p_0, w_1, \delta_1, p_1)\ldots(p_{n-1}, w_n, \delta_n, p_n)\in\pathsof{\avass}$ is the sum of all induced counter changes $\sum_{1\leq i\leq n}\delta_{n}$. 
%
\ekmark{If the VASS is defined on the dyck alphabet $\Sigma_{n}=\setcond{a_i, \bar{a}_i}{i<n}$, we extend this to the external counters by $\balanceof{\apath}=\sum_{1\leq i\leq n}\balanceof{w_i}$ as well.
%
We write $\allbalanceof{\apath}$ to denote the $d+n$ dimensional vector $(\vassbalanceof{\apath}, \balanceof{\apath})$.}




Recall that configurations of the B\"uchi VASS $\avass$ are elements of the set $Q\times\mathbb{N}^d$.
%
We call the second component in a configuration the \emph{counter valuation}
and refer to the $i$th entry as the \emph{value of counter $i$}.
%
Moreover we also consider a set of \emph{extended configurations} $\states\times\natomega^{d}$,
where $\natomega = \N \cup \{\omega\}$.
%
Here $\omega$ is used to represent a counter value that has become unbounded.
%
For an extended configuration $(q,\bmm)$ we use $\omega(q,\bmm) \subseteq [1,d]$ to denote the
set of counters valued $\omega$ in $\bmm$.
%
Comparisons and arithmetic operations between integer values and $\omega$ behave as expected,
treating $\omega$ as $\infty$.
%
Our definitions of runs, paths, loops, etc.\ carry over to \emph{extended} versions over
the set of extended configurations in a straightforward way.




==> quant-elim.tex <==
%

\subsection{Definitions and Main Theorem}

Given a rational number $r \in \Q$ we say $r$ \emph{has complexity} $c$
if there are numbers $p \in \Z, q \in \N$ with $r = \frac{p}{q}$ and $|p|,|q| \leq r$.
Intuitively, $r$ requires $\sim \log_2 c$ bits to write down,
and furthermore, $|p| < c$ implies $|r| < c$.
We say a vector in $\Q^n$ or a matrix in $\Q^{m \times n}$ has complexity $c$
if all of its entries have complexity $c$.

Let $\bA(t) \in \Z[t]^{m \times n}$ be a matrix with $m$ rows and $n$ columns
over the set of polynomials in variable $t$ with integer coefficients,
and let $\bb \in \Z[t]^m$ be an $m$-dimensional column vector over the same set.
Consider the system of inequalities $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$
with possible solutions $t \in \Q$, $\bx \in \Q^n$.
If such solutions exist, then we call $\cS$ \emph{feasible}.

We use $\deg\cS$ to denote the highest degree of a polynomial appearing in $\cS$,
$\maxc\cS$ to denote the maximum absolute value of a coefficient
appearing amongst the polynomials in $\cS$.
The values $\deg\bA$, $\deg\bb$, $\maxc\bA$, and $\maxc\bb$ for matrices and vectors
are defined analogously.

\begin{theorem}\label{old-solution-size}
  Let $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$ be a system of inequalities with
  $\bA(t) \in \Z[t]^{m \times n}$ and $\bb \in \Z[t]^m$.
  If $\cS$ is feasible, then there are solutions $t \in \Q$, $\bx \in Q^n$ such that
  $t$ and $\bx$ have complexity $(\deg\cS \cdot \maxc\cS)^{O(\deg\cS^3 \cdot n^5)}$
\end{theorem}

In particular \cref{old-solution-size} shows that a feasible system $\cS$
always has solutions of at most singly exponential size.
The main ingredient required to prove \cref{old-solution-size} is the following:

\begin{lemma}\label{old-exist-solutions-size}
  Consider a feasible system of inequalities $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$ with
  $\bA(t) \in \Z[t]^{m \times n}$ and $\bb \in \Z[t]^m$.
  Then the existentially quantified system $\exists \bx \in \Q^n\colon \cS$ has a solution
  $t \in \Q$ of complexity $(\deg\cS \cdot \maxc\cS)^{O(\deg\cS^2 \cdot n^4)}$.
\end{lemma}

In the following we shorten $\exists \bx \in \Q^n\colon \cS$ to $\exists \bx\colon \cS$,
since the solution space for $\cS$ is clear from context.
Let us now explain how to prove \cref{old-solution-size} assuming \cref{old-exist-solutions-size} holds:

\begin{proof}[Proof of \cref{old-solution-size}]
  Let $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$ be a feasible system of inequalities.
  We apply \cref{old-exist-solutions-size} to obtain a solution $t \in \Q$
  to the existentially quantified system $\exists \bx\colon \cS$.
  By \cref{old-exist-solutions-size} and the definition of complexity,
  there are numbers $p \in \Z, q \in \N$ with $t = \frac{p}{q}$ and
  $|q|,|p| \leq (\deg\cS \cdot \maxc\cS)^{O(\deg\cS^2 \cdot n^4)}$.
  If we instantiate $\cS$ with solution $\frac{p}{q}$, we obtain a system with rational coefficients,
  where $q^{\deg\cS}$ is the least common denominator.
  Therefore we can define $\bB = q^{\deg\cS} \bA(\frac{p}{q})$ and $\bd = q^{\deg\cS} \bb(\frac{p}{q})$
  to obtain the system $\cT := \bB \bx \geq \bd \wedge \bx \geq 0$ of linear inequalities
  with integer coefficients.
  Clearly a solution $\bx$ of $\cT$ also is a solution of $\cS$ instantiated with $\frac{p}{q}$
  and vice-versa.
  
  Regarding the size of the system $\cT$, we get
  \begin{align*}
    \maxc\bB &\leq \maxc\bA \big((\deg\cS \cdot \maxc\cS)^{O(\deg\cS^2 \cdot n^4)}\big)^{\deg\cS}\\
    &\leq (\deg\cS \cdot \maxc\cS)^{O(\deg\cS^3 \cdot n^4)},
  \end{align*}
  and similarly, $\maxc\bd \leq (\deg\cS \cdot \maxc\cS)^{O(\deg\cS^3 \cdot n^4)}$.
  Using bounds on short integer solutions for such systems
  we obtain a solution $\bx$ to $\cT$ of complexity $(\deg\cS \cdot \maxc\cS)^{O(\deg\cS^3 \cdot n^5)}$
\end{proof}


\subsection{Eliminating the Quantifier}

Towards a proof of \cref{old-exist-solutions-size} we would like to simplify the system
$\exists \bx \colon \cS$.
To this end we eliminate the quantifier $\exists \bx$ to obtain a boolean combination $\Phi(t)$
of polynomial inequalities that are only dependent on a possible solution $t$.
Here we extend the notation $\maxc \pi$ and $\deg \pi$ to singular polynomials $\pi(t) \in \Q[t]$.

\begin{lemma}\label{old-system-to-formula}
  Let $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$ be a system of inequalities with
  $\bA(t) \in \Z[t]^{m \times n}$ and $\bb \in \Z[t]^m$. 
  Then there is a finite set of indices $I \subseteq \N$,
  and for each $i \in I$ there is a finite set of polynomials $\Pi_i \subseteq \Z[t]$ with
  $\deg\pi \leq O(n \cdot \deg\cS)$ and $\maxc\pi \leq (\deg\cS \cdot \maxc\cS)^{O(n^2)}$
  for each $\pi \in \bigcup_{i \in I} \Pi_i$, such that the following holds:
  A number $t \in \Q$ is a solution to the system $\exists \bx\colon \cS$
  if and only if $t$ satisfies the formula $\Phi(t)$,
  where $\Phi(t) := \bigvee_{i \in I} \bigwedge_{\pi \in \Pi_i} \pi(t) \sqsupset_{i,\pi} 0$
  with $\sqsupset_{i,\pi} \in \{\geq, >\}$ for each $i \in I$ and $\pi \in \Pi_i$.
\end{lemma}

\begin{proof}
  Consider the matrix
  $\bD(t) := \left(\begin{aligned}&\bA(t)\\&\bI_n\end{aligned}\right) \Z[t]^{(m + n) \times n}$,
  constructed by glueing the $n \times n$ identity matrix $\bI_n$ to the bottom of $\bA(t)$.
  Similarly, consider the vector 
  $\bc(t) := \left(\begin{aligned}&\bb(t)\\&\bzero_n\end{aligned}\right) \Z[t]^{m + n}$
  constructed by extending $\bb(t)$ with $n$ zeroes.
  Then we can equivalently rewrite the system $\cS$ as $\cS' := \bD(t) \bx \geq \bc(t)$.
  Given a set of row numbers $R \subseteq [1,m+n]$ we use $\bD_R(t) \in \Z[t]^{|R| \times n}$
  to denote the matrix obtained from $\bD(t)$ by deleting all other rows.
  We extend this notation to $\bc_R(t) \in \Z[t]^{|R|}$ obtained from the vector $\bc(t)$.
  From linear programming we know that $t \in \Q$ is a solution to $\cS'$
  if and only if $t$ satisfies the following formula:
  \[
    \bigvee_{R \subseteq [1,m+n], |R| = n} \det \bD_R(t) \neq 0
    \wedge \bD(t) \cdot \bD_R(t)^{-1} \cdot \bc_R(t) \geq \bc,
  \]
  where $\det$ denotes the matrix \emph{determinant}.
  We would like to bring this formula into the required form for $\Phi(t)$.
  Recall that given an invertible matrix $\bC$, we can compute its inverse as
  $\bC^{-1} = \frac{\adj \bC}{\det \bC}$, where $\adj$ denotes the \emph{adjugate} matrix.
  Now if we perform a case split of $\det \bD_R(t) \neq 0$ into $> 0$ and $< 0$ in the above formula,
  and then multiply by $\det \bD_R(t)$ we get the following:
  \begin{align*}
    \bigvee_{R \subseteq [1,m+n], |R| = n}~
    &\left( \begin{aligned}
      &\det \bD_R(t) > 0 \\
      &\wedge \bD(t) \cdot \adj\bD_R(t) \cdot \bc_R(t) \geq \det \bD_R(t) \cdot \bc
    \end{aligned} \right) \\
    &\vee \left( \begin{aligned}
      &\det \bD_R(t) < 0 \\
      &\wedge \bD(t) \cdot \adj\bD_R(t) \cdot \bc_R(t) \leq \det \bD_R(t) \cdot \bc
    \end{aligned} \right)
  \end{align*}
  If we consider each matrix inequality in this formula to be a conjunction of the
  inequalities given by each individual row, then we can rewrite it into a formula of the form
  $\Phi(t)' := \bigvee_{i \in I} \bigwedge_{(\pi,\pi') \in \Pi'_i} \pi(t) \sim_{i,(\pi,\pi')} \pi'(t)$,
  where $I$ is a finite set of indices, the $\Pi'_i$ are finite sets of pairs of polynomials,
  and the $\sim_{i,(\pi,\pi')}$ are relations in $\{\geq,>,\leq,<\}$.
  By subtracting $\pi'(t)$ from each inequality and multiplying by $-1$ as necessary, we obtain
  a formula $\Phi(t)$ of the required form.
  
  It remains to argue that the polynomials in $\Phi(t)$
  have the required degree and maximum absolute value amongst their coefficients.
  Since all the exponents and absolute values of coefficients are already present
  in the previous formula, it suffices to compute these values for 
  $\det \bD_R(t)$, $\bD(t) \cdot \adj\bD_R(t) \cdot \bc_R(t)$, and $\det \bD_R(t) \cdot \bc$
  for all $R$.
  Let $S_n$ be the set of all permutations of $[1,n]$, and let
  $d_{R,i,j}(t)$ be the entry in the $i$th row and $j$th column of $\bD_R(t)$.
  One way to compute the latter's determinant is
  $\det \bD_R(t) = \sum_{\sigma \in S_n} \sgn{\sigma} \prod_{i = 1}^n d_{R,i,\sigma(i)}$.
  Hence, $\deg \det \bD_R(t) \leq n \cdot \deg \bD_R(t) \leq n \cdot \deg \cS'$.
  Regarding $\maxc$, note that each polynomial $d_{R,i,j}(t)$ is an additive term of
  at most $\deg \bD_R(t) + 1$ monomials, each with a potentially large coefficient,
  and further note that $|S_n| = n!$.
  Therefore:
  \begin{align*}
    \maxc \det \bD_R(t)~ &\leq n!\big((\deg \bD_R(t)+1) \cdot \maxc \bD_R(t)\big)^n \\
    &\leq 2^{n \log_2 n} \cdot (\deg \cS'+1)^n \cdot (\maxc \cS')^n\\
    &\leq (\deg \cS' \cdot \maxc \cS')^{O(n^2)}.
  \end{align*}
  Recall that each entry of the adjugate $\adj\bD_R(t)$ can be computed by deleting
  one row and one column from $\bD_R(t)$ and computing the determinant of the resulting matrix.
  This implies $\deg \adj \bD_R(t) \leq \deg \det \bD_R(t)$ and
  $\maxc \adj \bD_R(t) \leq \maxc \det \bD_R(t)$, and therefore:
  \begin{align*}
    \deg (\bD(t) \cdot \adj\bD_R(t) \cdot \bc_R(t))~
    &\leq \deg \cS' + n \cdot \deg \cS' + \deg \cS' \\
    &= (n + 2) \cdot \deg \cS' = O(n \cdot \deg \cS'),
  \end{align*}
  For $\maxc$ we again remark that each polynomial is comprised of $\deg + 1$ monomials,
  and further that computing each entry per matrix multiplication here involves adding up $n$ terms.
  Thus, we get
  \begin{align*}
    &\maxc(\bD(t) \cdot \adj\bD_R(t) \cdot \bc_R(t)) \\
    &~\begin{aligned}
      \leq~ & (\deg\bD(t) \cdot \maxc\bD(t)) \cdot n \cdot (\deg\adj\bD_R(t) \cdot \maxc\adj\bD_R(t)) \\
      &\cdot n \cdot (\deg\bc_R(t) \cdot \maxc\bc_R(t)) \\
      \leq~ & \deg\cS' \cdot \maxc\cS' \cdot n \cdot O(n \cdot \deg S')
      \cdot (\deg \cS' \cdot \maxc \cS')^{O(n^2)} \\
      &\cdot n \cdot \deg\cS' \cdot \maxc\cS' \\
      =~ & O\big(n^3 \cdot (\deg S')^3 \cdot (\maxc S')^2\big)
      \cdot (\deg \cS' \cdot \maxc \cS')^{O(n^2)}\\
      =~ & (\deg \cS' \cdot \maxc \cS')^{O(n^2)}
    \end{aligned}
  \end{align*}
  Finally,
  $\deg (\det \bD_R(t) \cdot \bc) \leq O(n \cdot \deg \cS') + \deg \cS' = O(n \cdot \deg \cS')$,
  and 
  \begin{align*}
    &\maxc(\det \bD_R(t) \cdot \bc)\\
    &~\leq (\deg \cS' \cdot \maxc \cS')^{O(n^2)} \cdot O(n \cdot \deg \cS')
    \cdot \maxc \cS' \cdot \deg \cS'\\
    &~= (\deg \cS' \cdot \maxc \cS')^{O(n^2)}.
  \end{align*}
  Since $\deg \cS' = \deg \cS$ and $\maxc \cS' = \maxc \cS$ by construction,
  we obtain the required values for polynomials appearing in $\Phi(t)$.
\end{proof}


\subsection{Root Separation}

Consider the \emph{roots} of a polynomial $\pi(t) \in \Z[t]$, formally defined as
$\Roots{\pi} := \{-\infty,\infty\} \cup \{t' \in \R \mid \pi(t') = 0\}$.
We include $-\infty$ and $\infty$ so that the entire set $\R$ decomposes into intervals
between adjacent roots of $\pi(t)$.
Additionally, we naturally extend this notation to sets of polynomials $\Pi(t) \subseteq \Z[t]$,
i.e.\ $\Roots{\Pi} := \bigcup_{\pi \in \Pi} \Roots{\pi}$.

\begin{lemma}\label{old-formula-to-roots}
  Let $I \subseteq \N$ be a finite set of indices,
  and for each $i \in I$ let $\Pi_i \subseteq \Z[t]$ be a finite set of polynomials,
  where $\Pi = \bigcup_{i \in I}\Pi_i$ is the finite union of these sets.
  Moreover let $\Phi(t)$ be a formula of the form
  $\Phi(t) := \bigvee_{i \in I}\bigwedge_{\pi \in \Pi_i} \pi(t) \sqsupset_{i,\pi} 0$,
  where $\sqsupset_{i,\pi} \in \{>,\geq\}$ for each $i \in I$ and $\pi \in \Pi_i$.
  
  Then there is a formula of the form
  $\Psi(t) := \bigvee_{j \in J} \ell_j \sqsubset_j t \sqsubset'_j u_j$;
  where $J \subseteq \N$ is a finite set of indices,
  $\ell_j, u_j \in \Roots{\Pi}$ for each $j \in J$,
  and $\sqsubset_j, \sqsubset'_j \in \{<, \leq\}$ for each $j \in J$;
  such that a number $t \in \Q$ satisfies $\Phi(t)$ if and only if $t$ satisfies $\Psi(t)$.
\end{lemma}

\begin{proof}
  Let $\pi(t) \in \Z[t]$ be a polynomial with $|\Roots{\pi}| = k$ and let
  $-\infty = r_1 < r_2 < \ldots < r_k = \infty$ be the ascending sequence of its roots.
  Then for each $i \in [1,k-1]$ clearly the interval $[r_i,r_{i+1}]$
  contains either no positive or no negative numbers.
  Now consider the inequality $\pi(t) \sqsupset 0$ with $\sqsupset\in \{>,\geq\}$.
  Clearly $t \in \Q$ satisfies this inequality if and only if
  $\bigvee_{1 \leq i < k, [r_i,r_{i+1}] \subseteq \R_0^+} r_i \sqsubset t \sqsubset r_{i+1}$,
  where $\sqsubset$ is the reverse of $\sqsupset$ and $\R_0^+$ denotes the non-negative real numbers.
  
  With the above we now have that $\Phi(t)$ is equivalent to a formula of the form
  $\Phi'(t) := \bigvee_{i \in I}\bigwedge_{\pi \in \Pi_i}
  \bigvee_{k \in K_\pi} \ell_{\pi,k} \sqsubset_{i,\pi} t \sqsubset_{i,\pi} u_{\pi,k}$,
  where $K_\pi \subseteq \N$ is a finite set of indices for each $\pi \in \Pi$,
  $\ell_{\pi,k}, u_{\pi,k} \in \Roots{\pi}$ for each $\pi \in \Pi$ and $k \in K_\pi$,
  and $\sqsupset_{i,\pi} \in \{<,\leq\}$ for each $i \in I$ and $\pi \in \Pi_i$.
  If we apply distributivity to the middle $\bigwedge$ and right $\bigvee$ in $\Phi'(t)$,
  we obtain another equivalent formula of the following form:
  $\Psi'(t) := \bigvee_{j \in J} \bigwedge_{k' \in K'_j}
  \ell_{j,k'} \sqsubset_{j,k'} t \sqsubset_{j,k'} u_{j,k'}$,
  where similar to before $J$ and all $K'_j$ are sets of indices,
  $\ell_{j,k'}, u_{j,k'} \in \Roots{\Pi}$, and $\sqsupset_{j,k'} \in \{<,\leq\}$.
  
  Finally, to satisfy $\Psi'(t)$, a number $t$ only has to adhere to the
  strictest upper and lower bound in each conjunction.
  Therefore, to construct an equivalent formula $\Psi(t)$ of the desired form,
  we define $\ell_j = \max_{k' \in K'_j} \ell_{j,k'}$ and $u_j = \min_{k' \in K'_j} u_{j,k'}$.
  Regarding the relation $\sqsubset_j$ in $\Psi(t)$, we pick $<$ if there is some $k \in K_j'$
  such that $\ell_j = \ell_{j,k'}$ and ${\sqsubset_{j,k'}} = {<}$, and we pick $\leq$ otherwise.
  The case of the relation $\sqsubset'_j$ for $u_j$ is analogous.
\end{proof}

We define $\Separation{\pi} := \min_{r \neq r' \in \Roots{\pi} \cap \R}|r-r'|$,
which evaluates to $\infty$ if $|\Roots{\pi} \cap \R| < 2$.

\begin{theorem}[Rump's Bound {\cite[Theorem 8.5.5]{Mishra93}}]\label{old-rumps-bound}
  Let $\pi(t) \in \Z[t]$ be a polynomial with $\deg\pi = \ell$.
  Then 
  \[ \Separation{\pi} > \frac{1}{\ell^{\ell+1}(1+ \|\pi\|_1)^{2\ell}}. \]
\end{theorem}

%

Note that $\|\pi\|_1 \leq (\deg\pi + 1) \cdot \maxc\pi$ for any polynomial $\pi$.
With this, we are finally ready to prove \cref{old-exist-solutions-size}.

\begin{proof}[Proof of \cref{old-exist-solutions-size}]
  Let $\cS := \bA(t) \bx \geq \bb(t) \wedge \bx \geq 0$ be a feasible system of inequalities with
  $\bA(t) \in \Z[t]^{m \times n}$ and $\bb \in \Z[t]^m$.
  Consider the existentially quantified system $\exists \bx \colon \cS$.
  If we apply both \cref{old-system-to-formula,old-formula-to-roots}, then these yield
  a finite set of polynomials $\Pi \subseteq \Z[t]$, and a formula
  $\Psi(t) := \bigvee_{j \in J} \ell_j \sqsubset_j t \sqsubset'_j u_j$;
  where $J \subseteq \N$ is a finite set of indices,
  $\ell_j, u_j \in \Roots{\Pi}$ for each $j \in J$,
  and $\sqsubset_j, \sqsubset'_j \in \{<, \leq\}$ for each $j \in J$.
  Furthermore we get that a number $t \in \Q$ is a solution to $\exists \bx \colon \cS$
  if and only if $\Psi(t)$ holds;
  and each polynomial $\pi \in \Pi$ exhibits bounds
  $\deg\pi \leq O(n \cdot \deg\cS)$ and $\maxc\pi \leq (\deg\cS \cdot \maxc\cS)^{O(n^2)}$.
  
  Since $\cS$ is feasible, there is an index $j \in J$
  such that the inequality $\ell_j \sqsubset_j t \sqsubset'_j u_j$ is feasible.
  We distinguish two cases regarding $\ell_j$ and $u_j$.
  In each case we look for a solution $t = \frac{p}{q}$,
  where $p \in \Z$ and $q \in \N \setminus \{0\}$,
  such that $t$ has the required complexity.
  
  \begin{description}
    \item[case $\bm{\ell_j = u_j}$:]
    Then ${\sqsubset_j} = {\sqsubset'_j} = {\leq}$, and $\frac{p}{q} = \ell_j = u_j$.
    Thus, there is a $\pi \in \Pi$ such that $\frac{p}{q} \in \Roots{\pi}$.
    Since also $\frac{p}{q} \in \Q$ we get that $p,q \leq \maxc\pi$
    using the Rational Root Theorem.
    \item[case $\bm{\ell_j < u_j}$:]
    If $\ell_j = -\infty, u_j = \infty$ then we can pick $p = 0, q = 1$ as a valid solution.
    Otherwise we assume $u_j \neq \infty$, with the case $\ell_j \neq -\infty$ being analogous.
    Then $\ell_j \in \Roots{\pi}$ and $u_j \in \Roots{\pi'}$ for some $\pi,\pi' \in \Pi$.
    Note that $\pi$ and $\pi'$ need not be the same polynomial.
    However, $\ell_j$ and $u_j$ are both roots of the product polynomial,
    i.e.\ $\ell_j, u_j \in \Roots{\pi_\times}$, where $\pi_\times = \pi\cdot\pi'$.
    Moreover, note that $\deg\pi_\times = \deg\pi \cdot \deg\pi'$ and
    $\|\pi_\times\|_1 \leq \|\pi\|_1 \cdot \|\pi'\|_1$.
    Therefore using Rump's Bound we get
    \begin{align*}
      |u_j - \ell_j|
      ~>~& \big(\deg\pi_\times^{\deg\pi_\times+1}
      \cdot (1+\|\pi_\times\|_1)^{2\deg\pi_\times}\big)^{-1}\\
      ~\geq~& \Big(O(n^2\cdot\deg\cS^2)^{O(n^2\cdot\deg\cS^2)} \cdot \Big(O(n^2\cdot\deg\cS^2)\\
      &\quad\cdot (\deg\cS \cdot \maxc\cS)^{O(n^2)}\Big)^{O(n^2\cdot\deg\cS^2)}\Big)^{-1}\\
      ~\geq~& \big((\deg\cS \cdot \maxc\cS)^{O(n^4\cdot\deg\cS^2)}\big)^{-1}.
    \end{align*}
    In the following we also use $B$ as a shorthand for
    $(\deg\cS \cdot \maxc\cS)^{O(n^4\cdot\deg\cS^2)}$.
    Immediately we get $B(u_j - \ell_j) > 1$.
    Thus, there is an integer $p \in \Z$ such that $B \ell_i < B u_j - 1 \leq p < B u_j$.
    Dividing by $B$ yields $\ell_i < \frac{p}{B} < u_j$, meaning we can choose a
    denominator $q \in \N \setminus \{0\}$ for a suitable solution with $q \leq B$.
    Finally, by Cauchy's bound on root sizes,
    we get
    \begin{align*}
      |u_j| \leq 1 + \|\pi'\|_1 \leq~ &O(n \cdot \deg\cS) \cdot (\deg\cS \cdot \maxc\cS)^{O(n^2)}\\
      \leq~ &(\deg\cS \cdot \maxc\cS)^{O(n^2)},
    \end{align*}
    and therefore $|p| \leq B|u_j| + 1 \leq B \cdot (\deg\cS \cdot \maxc\cS)^{O(n^2)}$.
    Due to $O$-notation, the second factor is subsumed by $B$ here.
  \end{description}
  In all cases $B = (\deg\cS \cdot \maxc\cS)^{O(n^4\cdot\deg\cS^2)}$
  is a bound on the complexity of $t$, as required.
\end{proof}


==> witness.tex <==
We feature a Rackoff inspired proof of \cref{Theorem:Bound}, which bounds the short inseparability blooms with stems.
%
The proof is structured similarly to \cite{Habermehl97}.
%
In \cite{Habermehl97}, the authors prove bounds on runs that cover a configuration they previously visited.
%
At each step of the proof, the authors use short solutions to systems of linear integer inequalities to shorten runs.
%
We intend to follow this approach.
%
However, there are two major problems we need to take care of.
%
First, inseparability flowers are expressed in terms of non-linear constraints.
%
For this reason, we need to use the bounds for short solutions of singly non-linear systems that we developped in \cref{section:quant-elim}.
%
Second, our bounds in \cref{section:quant-elim} are 
on rational solutions, not integer solutions.
%
We need to construct our (in)equation systems in a way that allows us to move from rational solutions to integer solutions.


For the rest of this section, fix an \ekmark{n-visible(?)} VASS $\avass=(\states, q_0, \Sigma_{n}, \transitions, \finalstates)$, with the set of combined counters $\combinedcounters=\set{0, \ldots, d+n-1}$.
%
We write $\nat^{\combinedcounters}$ and $\natomega^{\combinedcounters}$ to denote the respective sets $\nat^{d+n}$ and $\natomega^{d+n}$.
%
For a set of counters $\omegacounters\subseteq\combinedcounters$ and a configuration $(q, \bmm)\in\states\times\natomega^{\combinedcounters}$, we write $(q, \bmm)^{\omegacounters}$ to denote the configuration $(q, \replacein{\bmm}{\omegacounters}{\omega})\in\states\times\natomega^{\combinedcounters}$.  


We develop a notion of extended blooms.
%
Intuitively, an extended bloom is a configuration with a path that leads to an inseparability bloom.
%
Let $\counters\subseteq\combinedcounters$ and $\combinedcounters=\omegacounters\uplus\counters$.
%
An extended bloom $W=((q, \bmm), \apath, \counters, \alpha, \beta, \gamma)$ consists of a start configuration $(q, \bmm)\in\states\times\nat^{\combinedcounters}$, a path $\apath\in\pathsof{\avass}$ with some $(\finalstate, \bmm_{f})\in\finalstates\times\nat^{\combinedcounters}$ where 
\begin{itemize}
    \item $\reachof{(q, \bmm)^{\omegacounters}}{\apath}$ covers $(\finalstate, \bmm_{f})^{\omegacounters}$
    \item $((\finalstate, \bmm_{f}), \counters, \alpha, \beta, \gamma)$ is an inseparability bloom.
\end{itemize}
%
Note that even with the initial path, the existence of an extended bloom from $(q_0, \zerovec)$ is not equivalent to the existence of an inseparability bloom with a stem.
%
This is because a stem has additional unboundedness conditions which may not be met by an extended bloom.
%
Nevertheless, a bound on the size of short extended blooms yields a bound on short inseparability blooms with stems.
%
We define the size of an extended bloom as $\sizeof{((q, \bmm), \apath, \counters, \alpha, \beta, \gamma)}=\sizeof{\apath}+\max(\sizeof{\alpha}, \sizeof{\beta}, \sizeof{\gamma})$.
%
We say that $((q, \bmm), \apath, \counters, \alpha, \beta, \gamma)$ is an extended bloom from $(q, \bmm)$.
%
Now let 
%
$$B_{\avass}=\max_{c\in\states\times\nat^{\combinedcounters}}\min\setcond{\sizeof{W}}{W\text{ extended bloom from }c}\in\natomega.$$

Our aim is to impose the following bound on $B_{\avass}$.
%
\begin{lemma}\label{Lemma:ShortIncWitness}
    $B_{\avass}\leq (2^{\sizeof{\avass}}\sizeof{\states})^{\sizeof{\combinedcounters}^{\bigoof{\sizeof{\combinedcounters}}}}$.
\end{lemma}

As we promised, this bound implies \cref{Theorem:Bound}.
%
\begin{proof}[Proof of \cref{Theorem:Bound}]
    Let $\abloom=((\finalstate, \bmm_{f}), \counters, \alpha, \beta, \gamma)$ be an inseparability bloom with a stem in $\avass$, and let $\combinedcounters=\counters\uplus\omegacounters$.
    %
    Then, $((\finalstate, \bmm_{f}), \varepsilon, \counters, \alpha, \beta, \gamma)$ is an extended bloom, as $\reachof{(\finalstate, \bmm_{f})^{\omegacounters}}{\varepsilon}$ covers $(\finalstate, \bmm_{f})^{\omegacounters}$ and $\abloom$ is an inseparability bloom.
    %
    We apply \cref{Lemma:ShortIncWitness} to get an extended bloom $((\finalstate, \bmm_{f}), \apath^{*}, \counters, \alpha^{*}, \beta^{*}, \gamma^{*})$ with 
    %
    $$\sizeof{\apath^{*}}+\max(\sizeof{\alpha^{*}}, \sizeof{\beta^{*}}, \sizeof{\gamma^{*}})\leq B_{\avass}.
    $$
    %
    Let $\reachof{(\finalstate, \bmm_{f})^{\omegacounters}}{\apath}=(\finalstate^{*}, \bmm_1)^{\omegacounters}$ for some $(\finalstate^{*}, \bmm_{1})\in\finalstates\times\nat^{\combinedcounters}$, where $((\finalstate^{*}, \bmm_{1}), \counters, \alpha^{*}, \beta^{*}, \gamma^{*})$ is an inseparability bloom.
    %
    Note that this inseparability bloom can still be very large, 
    since we did not bound the size of the configuration.
    %
    Towards a bound on the configuration, let $\bmm^{*}\in\nat^{\combinedcounters}$ with $\bmm^{*}[i]=\min(\bmm_{1}[i], 2^{\sizeof{\avass}} B_{\avass})$ for all $i\in\combinedcounters$.
    %
    We argue that taking any prefix of $\alpha^{*}$, $\beta^{*}$, and $\gamma^{*}$ from $(\finalstate^{*}, c^{*})$ reaches a configuration with a positive value on counter $i\in\counters$.
    %
    Let $i\in\counters$ with $\bmm^{*}[i]\leq 2^{\sizeof{\avass}} B_{\avass}$, we know $\bmm^{*}[i]=\bmm_{1}[i]$.
    %
    By the definition of the inseparability bloom, the prefixes of loops already remain positive on counter $i$, starting from $\bmm_{1}[i]$.
    %
    Now let $i\in\counters$ with $\bmm^{*}[i]> 2^{\sizeof{\avass}} B_{\avass}$.
    %
    We know $\sizeof{\alpha^{*}}, \sizeof{\beta^{*}}, \sizeof{\gamma^{*}}\leq B_{\avass}$. 
    %
    Since each transition can take at most $2^{\sizeof{\avass}}$ tokens away from a counter, the counter value can decrease by at most $2^{\sizeof{\avass}}B_{\avass}$ tokens along any of these loops.
    %
    The bound $\bmm^{*}[i]> 2^{\sizeof{\avass}} B_{\avass}$, ensures that the counter $i$ remains positive.
    %
    Then, $\abloom^{*}=((\finalstate^{*}, \bmm^{*}), \counters, \alpha^{*}, \beta^{*}, \gamma^{*})$ is an inseparability bloom with $\sizeof{\abloom^{*}}\leq \bigoof{2^{\sizeof{\avass}} B_{\avass}}$.
    %
    \ekmark{This is readily the size bound in \cref{Theorem:Bound}.}
    %
    Finally we argue that $\abloom^{*}$ has a stem.
    %
    Because $\abloom$ is an inseparability flower, $(\finalstate, \replacein{\bmm_{f}}{\omegacounters}{k})$ is coverable for all $k\in\nat$.
    %
    Since taking $\apath$ from $(\finalstate, \bmm_{f})^{\omegacounters}$ reaches $(\finalstate^{*}, \bmm_{1})^{\omegacounters}$, we know that $(\finalstate^{*}, \replacein{\bmm_{1}}{\omegacounters}{k})$ is also coverable for all $k\in\nat$.
    %
    Finally, we have $\bmm_{1}\geq \bmm^{*}$.
    %
    Then, $(\finalstate^{*}, \replacein{\bmm^{*}}{\omegacounters}{k})$ is coverable for all $k\in\nat$ as well.
    %
    This concludes the proof.
\end{proof}

Now we show \cref{Lemma:ShortIncWitness}.
%
In order to do so, we define the concept of $r$-bounded and $\countersp$-repeating extended blooms.
%
An extended bloom $((q, \bmm), \apath, \counters, \alpha, \beta, \gamma)$ is $r$-bounded and $\countersp$-repeating where $r\in\nat$, $\countersp\subseteq\combinedcounters$, if the following three conditions hold for all $i\in\counters$ and $j\in\countersp$
\begin{itemize}
    \item $\reachof{(q, \bmm)^{\omegacounters}}{\apath'}=(q', \bmm')^{\omegacounters}$, with $\bmm'[i]\leq r$ for all $\apath'\in\prefix(\apath)$
    \item  $\reachof{(q_f, \bmm_f)}{\xi'}=(q'', \bmm'')$ where we also have that $\reachof{(q,\bmm)}{\apath}=(q_f, \bmm_f)$ with $\bmm''[i]\leq r$ for all prefixes $\xi'$ of $\alpha$, $\beta$, or $\gamma$
    \item $\allbalanceof{\apath}[j]\geq 0$.
\end{itemize}
%
Intuitively, $r$-bounded means that during the execution of $\apath.\alpha.\beta.\gamma$ from $(q, \bmm)$, counters in $\counters$ never go above $r$, and $\countersp$-repeating meains that the loops must have a positive effect on counters in $\countersp$.
%
Note that by the definition of an extended bloom, the counters in $\counters$ are guaranteed to remain positive while executing $\apath.\alpha.\beta.\gamma$ from $(q,\bmm)$.

We prove the following lemma, which is the key to the proof of \cref{Lemma:ShortIncWitness}.
%
As alluded to, this is where we use short solutions to Singly Non-Linear Systems.
%
The lemma is the analogue of \cite[Lemma 3.2]{Habermehl97}.

\begin{lemma}\label{Lemma:RBoundedWitnesses}
    Let $W$ be an extended bloom from $(q, \bmm)$ that is $r$-bounded and $\countersp$-increasing. 
    %
    Then, there is an $r$-bounded, $\countersp$-increasing extended bloom $W^{*}$ from $(q, \bmm)$ with $\sizeof{W^{*}}\leq (2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}$.
\end{lemma}

\begin{proof}
    Let $\counters, \countersp\subseteq\combinedcounters$, $r\in\nat$, $\combinedcounters=\counters\uplus\omegacounters$, and 
    $((q, \bmm), \apath, \counters, \alpha, \beta, \gamma)$ be an $r$-bounded, $\countersp$-repeating extended bloom.
    %
    Let $\reachof{(q, \bmm)^{\omegacounters}}{\apath}=(\finalstate, \bmm_f)^{\omegacounters}$ for some $(\finalstate, \bmm_{f})\in\finalstates\times\nat^{\combinedcounters}$, where $((\finalstate, \bmm_{f}), \counters, \alpha, \beta, \gamma)$ is an inseparability bloom. 
    %
    As in the proof of \cite[Lemma 3.2]{Habermehl97}, we can eliminate the loops that repeat the control state and the counter valuations of $\counters$ counters along the run of $(q, \bmm)^{\omegacounters}.\apath$.
    %
    Because there are $r$ possible values per counter $i\in\counters$, this gives us a new path $\apath_{1}$ that also has $\reachof{(q, \bmm)^{\omegacounters}}{\apath_{1}}=(\finalstate, \bmm_{f})^{\omegacounters}$ with $\sizeof{\apath_{1}}\leq r^{\sizeof{\counters}}\sizeof{\states}\leq r^{\sizeof{\combinedcounters}}\sizeof{\states}$.
    %
    To shorten $\alpha$, $\beta$, $\gamma$, we take the same approach as in \cite[Lemma 3.2]{Habermehl97}.
    %
    For each $\xi\in\set{\alpha, \beta, \gamma}$, we decompose $\xi$ into $\xi_{0}, \xi_{1}, \ldots \xi_{u}\in\loopsof{\avass}$ where $(q_f, \bmm_f)^{\omegacounters}.\xi_{0}$ visits the same configurations as $(q_f, \bmm_f)^{\omegacounters}.\xi$ does, and $\xi_{1}, \ldots, \xi_{u}$ are loops we eliminate from $\xi$ that do not repeat configurations (except at the beginning resp. the end).
    %
    The sizes $\sizeof{\xi_{0}}, \sizeof{\xi_{1}}, \ldots, \sizeof{\xi_{u}}$ are bounded from above by $\sizeof{\states}\cdot r^{\sizeof{\combinedcounters}}$.
    %
    Furthermore, since $(q_f, \bmm_f)^{\omegacounters}.\xi_{0}$ visits all the states and valuations of $\counters$ counters $(q_f, \bmm_f)^{\omegacounters}.\xi$ does, we can glue repetitions of $\xi_{0}, \ldots, \xi_{u}$ to get a loop $\xi'$ that (1) remains positive in $\counters$ counters and (2) has the same effect as $\xi$.
    %
    Let $\bx\in\nat^{u+1}$ and $\xi_{\bx}$ be the loop obtained by glueing $\bx[i]$ iterations of the loop $\xi_{i}$ together for all $i\leq u$.
    %
    Then, for $\bx_{\alpha},\bx_{\beta},\bx_{\gamma}\in\nat^{u+1}$,  $((\finalstate', \bmm'), \counters, \alpha_{\bx_{\alpha}}, \beta_{\bx_{\beta}}, \gamma_{\bx_{\gamma}})$ is an inseparability bloom, if 
    $\alpha_{\bx_{\alpha}}$, $\beta_{\bx_{\beta}}$, $\gamma_{\bx_{\gamma}}$ fulfill the last three conditions of an inseparability bloom.
    %
    This means that $((q_f, \bmm_f), \apath_{1}, \counters, \alpha_{\bx_{\alpha}}, \beta_{\bx_{\beta}}, \gamma_{\bx_{\gamma}})$ is an extended bloom.
    %
    Note that aside from positivity on $\counters$ counters, all the conditions for an inseparability bloom and being $\countersp$-repeating, are based on the vectors $\allbalanceof{\alpha_{\bx_{\alpha}}}$, $\allbalanceof{\beta_{\bx_{\beta}}}$, $\allbalanceof{\gamma_{\bx_{\gamma}}}$.
    %
    So, we can express the conditions for an inseparability bloom in terms of a singly non-linear system.
    %
    For the sake of efficiency, we assume that $\xi_{0}, \ldots, \xi_{u}$ only contains loops $\xi_{i}$ with different effects $\allbalanceof{\xi_{i}}$.
    %
    Elimination of the loops with duplicate effects does not make a difference. 
    %
    As we argued above, the only conditions we need to meet are based on the total effect.
    %
    Then, since $\sizeof{\xi_{i}}\leq \sizeof{\states}r^{\sizeof{\combinedcounters}}$, there can be at most $2\cdot 2^{\sizeof{\avass}}\sizeof{\states}r^{\sizeof{\combinedcounters}}$ different effects for each counter, giving us $u+1\leq(2^{\sizeof{\avass}+1}\sizeof{\states}r^{\sizeof{\combinedcounters}})^{\sizeof{\combinedcounters}}\leq (2^{\sizeof{\avass}}\sizeof{\states}r)^{\sizeof{\combinedcounters}^{2}}$.
    %
    With this at hand, we state the singly non-linear system that captures the inseparability bloom conditions, where 
    $\valuevec_{\xi}=\sum_{i\leq u}\bx_{\xi}[i]\cdot \loopvector_{\xi}[i]$ and $\loopvector_{\xi}=(\allbalanceof{\xi_{0}}, \ldots, \allbalanceof{\xi_{u}})$ for all $\xi\in\set{\alpha, \beta, \gamma}$, 
    \begin{itemize}
        \item $\bx_{\alpha}[0], \bx_{\beta}[0], \bx_{\gamma}[0]\geq 1$
        \item $(\valuevec_{\alpha}+ \valuevec_{\beta}+\valuevec_{\gamma})[i]\geq 0$, for all $i<d$
        \item $(\valuevec_{\alpha}+ \valuevec_{\beta})[i]\geq 0$, for all $i\in\set{d, \ldots, d+n-1}$
        \item $(\valuevec_{\alpha}+\valuevec_{\beta}+\valuevec_{\gamma}-t\cdot\valuevec_{\alpha})[i]=0$, for all $i\in\set{d, \ldots, d+n-1}$
        \item $\valuevec_{\alpha}[i], \valuevec_{\beta}[i], \valuevec_{\gamma}[i]\geq 0$, for all $i\in\countersp$
        \item $\bx_{\alpha}, \bx_{\beta}, \bx_{\gamma}\geq \zerovec$.
    \end{itemize}
    The first point states that the base loops, $\alpha_{0}, \beta_{0}, \gamma_{0}$, are taken at least once, and the 
    following three conditions are the conditions for an inseparability bloom, written in terms of loop effects.
    %
    Positivity ensures that no loop is ``taken'' a negative amount of times.
    %
    We direct the attention of the reader to the fact that, in contrast to \cite{Habermehl97}, we allow the base loops $\alpha_{0}$, $\beta_{0}$, $\gamma_{0}$, to be repeated as well.
    %
    The reason is that \cref{solution-size} only gives us rational solutions, while we need integer solutions.
    %
    By allowing this repetition, we keep the system homogenous aside from the first three conditions.
    %
    Then, if $(\bx_{\alpha}, \bx_{\beta}, \bx_{\gamma})$ is a solution, then so is $(k\bx_{\alpha}, k\bx_{\beta}, k\bx_{\gamma})$ for any $k\in\nat$.
    %
    This also holds for the first the first three constraints, albeit with the additional requirement $k\geq 1$.
    %
    So, if we are given a rational solution, we can multiply it by the common denominator to get an integer solution.
    %
    We invoke \cref{solution-size}.
    %
    Before we state the bound, we analyze the complexity of our system.
    %
    Our system has at most $5\sizeof{\combinedcounters}$ rows and at most $(2^{\sizeof{\avass}}\sizeof{\states}r)^{\sizeof{\combinedcounters}^{2}}$ columns.
    %
    The degree of the system is $1$.
    %
    The largest coefficient is bounded from above by the largest possible loop effect, $2^{\sizeof{\avass}}\sizeof{\states}r^{\sizeof{\combinedcounters}}$ as we argued above.
    %
    Then, \cref{solution-size} gives us rational $\bx_{\alpha}$, $\bx_{\beta}$, $\bx_{\gamma}$ and $K$, where $\bx_{\xi}[i]=\dfrac{p}{K}$ with 
    %
    $$|p|\leq (2^{\sizeof{\avass}+1}\sizeof{\states}r^{\sizeof{\combinedcounters}})^{\bigoof{\sizeof{\combinedcounters}^{5}}}\leq (2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}.$$
    %
    We have already argued that the integer vectors $K\bx_{\alpha}$, $K\bx_{\beta}$, $K\bx_{\gamma}$ are also solutions.
    %
    Let $\alpha^{*}$, $\beta^{*}$, and $\gamma^{*}$ be the loops we get by gluing the decomposed loops as directed by $K\bx_{\alpha}$, $K\bx_{\beta}$, $K\bx_{\gamma}$.
    %
    Because each coordinate of these vectors is smaller than 
    $(2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}$, and we have at most $(2^{\sizeof{\avass}}\sizeof{\states}r)^{\sizeof{\combinedcounters}^{2}}$ many loops with maximal size $\sizeof{\states}r^{\sizeof{\combinedcounters}}$, we get 
    \begin{align*}
        \sizeof{\xi^{*}}&\leq (2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}\cdot (2^{\sizeof{\avass}}\sizeof{\states}r)^{\sizeof{\combinedcounters}^{2}}\cdot \sizeof{\states}r^{\sizeof{\combinedcounters}}\\
        &=(2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}.
    \end{align*}
    %
    for all $\xi\in\set{\alpha, \beta, \gamma}$.

    Using the size bound on $\apath_{1}$, we bound the size of the $r$-bounded, $\countersp$-repeating extended bloom $W^{*}=((q,\bmm),\apath_{1}, \counters, \alpha^{*}, \beta^{*}, \gamma^{*})$ by 
    \begin{align*}
        \sizeof{W^{*}}\leq (2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}+\sizeof{\states}r^{\sizeof{\combinedcounters}}=(2^{\sizeof{\avass}}\sizeof{\states}r)^{\bigoof{\sizeof{\combinedcounters}^{6}}}.
    \end{align*}
    %
    This concludes the proof.
\end{proof}

We conclude this section by an argument for \cref{Lemma:ShortIncWitness}.
%
As the proof is the largely similar to \cite[Lemma 3.4]{Habermehl97}, the details have been moved to the appendix.
%
Towards an induction argument, we introduce the functions $f:\set{0, \ldots, \sizeof{\combinedcounters}-1}\to\nat$ and $g:\mathbb{P}(\combinedcounters)\times\mathbb{P}(\combinedcounters)\times(\states\times\nat^{\sizeof{\combinedcounters}})\to\nat$, where 
\begin{align*}
    g(\counters, \countersp, c)&=\min\setcond{\sizeof{W}}{W=(c, \apath, \counters, \alpha, \beta, \gamma)\text{ is a }\countersp\text{-increasing extended bloom from }c}\\
    f(h)&=\max_{c\in\states\times\nat^{\combinedcounters}}\max_{\countersp\subseteq\combinedcounters}\max_{\sizeof{\counters}=h}\; g(\counters, c).
\end{align*}
%
We bound $f(h)$ by \cref{Lemma:ShortParWitness}.
%
This also shows \cref{Lemma:ShortIncWitness}, since $B_{\avass}\leq \max\setcond{f(h)}{0\leq h\leq \sizeof{\combinedcounters}}$ and the bound is increasing.
%
\begin{lemma}\label{Lemma:ShortParWitness}
    $f(h)\leq (2^{\sizeof{\avass}}\sizeof{\states})^{\sizeof{\combinedcounters}^{\bigoof{h}}}$
\end{lemma}
%
Let $l=2^{\sizeof{\avass}}$.
%
It suffices to show that $f(h+1)\leq (l^{2}\sizeof{\states}\cdot f(h))^{\bigoof{\sizeof{\combinedcounters}^{6}}}$, and $f(0)\leq (l^{2}\sizeof{\states})^{\bigoof{\sizeof{\combinedcounters}^{6}}}$ to prove \cref{Lemma:ShortParWitness}.
%
This implies $f(h)=(l \sizeof{\states})^{\sizeof{\combinedcounters}^{\bigoof{h}}}$ by a standard induction, which proves our claim.
%
We sketch out the argument for the proof of \cref{Lemma:ShortParWitness}.
%
The proof is by induction on $h$.
%
We are given $\counters, \countersp\subseteq\combinedcounters$ and $c\in\states\times\nat^{\combinedcounters}$ with $\sizeof{\counters}=h$.
%
We assume that there is an extended bloom $W$ from $c$ that is $\countersp$-increasing.
%
We proceed by making a case distinction along whether 
$W$ is $l\cdot f(h)$-bounded.
%
If it is, we conclude with \cref{Lemma:RBoundedWitnesses}.
%
This also covers the base case.
%
If it is not, then one counter $i\in\counters$ exceeds $l\cdot f(h)$, and is followed by an extended bloom with one less counter whose positivity is tracked.
%
In this case, we get an extended bloom of size at most $f(h)$ using the induction hypothesis, and argue that the bloom also remains positive in counter $i$, as its initial value exceeded $l\cdot f(h)$.

\begin{comment}
    For coverability languages of VASS, the optimal algorithm is often \cite{Rackoff78,Habermehl97, stuffaboutunboundedness} based on short witnesses.
    %
    If a witness (e.g. a run) for some property is to be searched in the configuration space of the VASS, a size bound is imposed for the shortest such witness.
    %
    Then, the algorithm non-deterministically explores witnesses up to this size and returns yes if one is found.
    %
    If no witness is found, the size bound guarantees that no witness exists.
    %
    Our algorithm for regular separability is based on the same approach.
    %
    We prove a doubly exponential size bound for shortest concrete inseparability flower in a VASS, and give an algorithm based on this bound.
    
    \begin{lemma}\label{Lemma:ShortWitness}
        Let $\avass$ be a VASS. If it has a concrete inseparability flower $((\finalstate, c), \counters, \alpha_{0}, \beta_{0}, \gamma_{0})$, then it has an inseparability flower $((\finalstate', c'), \counters, \alpha, \beta, \gamma)$ with $\setcond{c'[i]}{i\in\combinedcounters}$ as well as the sizes of $\alpha$, $\beta$, $\gamma$ bounded from above by $\sizeof{\avass}^{2^{\bigoof{\sizeof{\combinedcounters}^b}}}$ for some $b$ independent of $\avass$.
    \end{lemma}
    
    This implies that the following non-deterministic, space bounded algorithm.
    %
    Let $\avass=(\states, q_0, \Sigma_{n}, \transitions, \finalstates)$.
    %
    Guess $(\finalstate, c)\in\states\times\nat^{\combinedcounters}$ with $c[i]\leq\sizeof{\avass}^{2^{\bigoof{\sizeof{\combinedcounters}^b}}}$ for all $i\in\combinedcounters$.
    %
    Using an unboundedness oracle, check that $(\finalstate, \replacein{c}{\counters}{k})$ is coverable for all $k\in\nat$ \cite{unboundednessref}.
    %
    Then guess three loops $\alpha$, $\beta$, $\gamma$ from $(\finalstate, c)$.
    %
    For each loop, keep the total effect of the loop, and the configuration it reaches from $(\finalstate, c)$ in memory.
    %
    This has exponentially many bits in $\sizeof{\avass}$.
    %
    Check whether $\alpha$, $\beta$, and $\gamma$ reach configurations that cover $(\finalstate, c)$, reject if not.
    %
    Finally, using the effects of the guessed loops $\allbalanceof{\alpha}$, $\allbalanceof{\beta}$, and $\allbalanceof{\gamma}$, verify the last three conditions of the concrete inseparability bloom using basic arithmetic operations.
    \end{comment}

